A Conditional Point Diffusion-Refinement Paradigm for 3D Point Cloud Completion

3D point cloud is an important 3D representation for capturing real world 3D objects. However, real-scanned 3D point clouds are often incomplete, and it is important to recover complete point clouds for downstream applications. Most existing point cloud completion methods use Chamfer Distance (CD) loss for training. The CD loss estimates correspondences between two point clouds by searching nearest neighbors, which does not capture the overall point density distribution on the generated shape, and therefore likely leads to non-uniform point cloud generation. To tackle this problem, we propose a novel Point Diffusion-Refinement (PDR) paradigm for point cloud completion. PDR consists of a Conditional Generation Network (CGNet) and a ReFinement Network (RFNet). The CGNet uses a conditional generative model called the denoising diffusion probabilistic model (DDPM) to generate a coarse completion conditioned on the partial observation. DDPM establishes a one-to-one pointwise mapping between the generated point cloud and the uniform ground truth, and then optimizes the mean squared error loss to realize uniform generation. The RFNet refines the coarse output of the CGNet and further improves quality of the completed point cloud. Furthermore, we develop a novel dual-path architecture for both networks. The architecture can (1) effectively and efficiently extract multi-level features from partially observed point clouds to guide completion, and (2) accurately manipulate spatial locations of 3D points to obtain smooth surfaces and sharp details. Extensive experimental results on various benchmark datasets show that our PDR paradigm outperforms previous state-of-the-art methods for point cloud completion. Remarkably, with the help of the RFNet, we can accelerate the iterative generation process of the DDPM by up to 50 times without much performance drop.

==> tables/multires+ablation_original.tex <==
%\setlength{\tabcolsep}{4.85pt}
\begin{table}[t!]
\vspace{-1em}
\parbox{0.49\columnwidth}{ 
        \centering
        \caption{Completion results on MVP dataset at the resolution of $4096, 8192, 16384$ points.}
        \label{tbl:multi_resolution_exps_on_mvp}
        \vspace{0.1em}
        \resizebox{0.49\columnwidth}{!}{
        \small{
    	\begin{tabular}{l | cc | cc | cc }
    		\Xhline{1pt}
    		\multirow{2}{*}{\# Points} & \multicolumn{2}{c|}{4096\Tstrut\Bstrut} & \multicolumn{2}{c|}{8192}    & \multicolumn{2}{c}{16384} \\
    		\cline{2-7}
    		& \scriptsize CD\Tstrut\Bstrut & \scriptsize F1 & \scriptsize CD & \scriptsize F1 & \scriptsize CD & \scriptsize F1 \\
    		\hline \hline
    		PCN\Tstrut       & 7.14       & 0.469       & 6.02 & 0.577                & 5.18        & 0.650       \\
    		TopNet           & 7.69       & 0.434       & 6.64 & 0.526                & 5.14        & 0.618       \\
    		FoldingNet       & 8.76       & 0.351       & 6.90  & 0.433               & 6.98        & 0.464     \\
    		MSN             & 5.37       & 0.583       & 4.40 & 0.663                & 4.09      &    0.696      \\
    		%
    		Cascade          & 5.46       & 0.579       & 4.51 & 0.686                & 3.90       & 0.743        \\
    		ECG              & 7.31       & 0.506       & 3.99 & 0.717                & 3.32       & 0.774      \\
    		GRNet            & 5.73       & 0.493       & 4.51 & 0.616                & 3.54        & 0.700       \\
    		%
    		PoinTr           & 4.29       & 0.638       & 3.52 & 0.725                & 2.95        & 0.783       \\
    		VRCNet\Bstrut    & 4.62       & 0.629       & 3.39 & 0.734                & 2.81        & 0.780       \\
    		\hline
    		Ours\Tstrut\Bstrut & \textbf{4.26} & \textbf{0.649} & \textbf{3.35} & \textbf{0.754} & \textbf{2.61} & \textbf{0.817} \\
    		\Xhline{1pt}
    	\end{tabular}
        }
        }
    }
    \hspace{0.03\columnwidth}
    \parbox{0.46\columnwidth}{ 
        \centering
        \caption{\small{Comparison of the coarse point clouds generated by different networks in DDPM. ``Aug.": Data augmentation. ``S(D).P.": Single(Dual)-path. 
        % ``D.P.": Dual-path.
        }}
        \label{tbl:ablation_on_mvp}
        \resizebox{0.46\columnwidth}{!}{
        \small{
        \begin{tabular}{l|c|ccc}
        	\Xhline{1pt}
        	Network \Tstrut\Bstrut & Aug. & \scriptsize CD & \scriptsize EMD & \scriptsize F1 \\ 
        	\hline \hline
        	Pointwise-net\Tstrut & \xmark  & 11.99 & 1.63 & 0.265\\
        	S.P. \PositionNet (G) & \xmark & 13.94 & 1.48 & 0.255\\
        	S.P. \PositionNet (C) & \xmark  & 10.78 & 1.54 & 0.382\\
        	D.P. PointNet++ & \xmark  & 9.39 & 1.38 & 0.355\\
        	Ours \Bstrut & \xmark & \textbf{8.71} & \textbf{1.29} & \textbf{0.389}\\
        	\hline
        	Pointwise-net\Tstrut & \cmark & 13.65 & 1.67 & 0.243\\
        	S.P. \PositionNet (G) & \cmark &  18.82 & 1.93 & 0.221\\
        	S.P. \PositionNet (C) & \cmark & 15.72 & 2.20 & 0.361\\
        	D.P. PointNet++ & \cmark & 12.49 & 1.74 & 0.352\\
        	Ours \Bstrut & \cmark & \textbf{10.52} & \textbf{1.43} & \textbf{0.407}\\
        	\Xhline{1pt}
        \end{tabular}
        }
        }
    }
\end{table}
